Beyond Role-Based Surgical Domain Modeling: Generalizable Re-Identification in the Operating Room

Surgical domain models improve workflow optimization through automated predictions of each staff member's surgical role. However, mounting evidence indicates that team familiarity and individuality impact surgical outcomes. We present a novel staff-centric modeling approach that characterizes individual team members through their distinctive movement patterns and physical characteristics, enabling long-term tracking and analysis of surgical personnel across multiple procedures. To address the challenge of inter-clinic variability, we develop a generalizable re-identification framework that encodes sequences of 3D point clouds to capture shape and articulated motion patterns unique to each individual. Our method achieves 86.19% accuracy on realistic clinical data while maintaining 75.27% accuracy when transferring between different environments - a 12% improvement over existing methods. When used to augment markerless personnel tracking, our approach improves accuracy by over 50%. Through extensive validation across three datasets and the introduction of a novel workflow visualization technique, we demonstrate how our framework can reveal novel insights into surgical team dynamics and space utilization patterns, advancing methods to analyze surgical workflows and team coordination.

==> highlights.tex <==



\item We propose a staff-centric approach to surgical domain modeling, characterizing individual and team dynamics over multiple surgical procedures.
\item The operating room domain is analyzed; we identify traits that introduce bias into methods modeling human motion.
\item A generalizable approach to OR re-identification is presented, leveraging 3D point cloud sequences to characterize the shape and articulated motion of individuals, mitigating texture bias in the OR.
\item We introduce person-specific 3D activity imprints and demonstrate their effectiveness in OR workflow analysis.



==> latexdiff_preamble.tex <==
\RequirePackage[normalem]{ulem}
\RequirePackage{color}
\definecolor{RED}{rgb}{1,0,0} %
\definecolor{BLUE}{HTML}{008080} %
\providecommand{\DIFadd}[1]{{\protect\color{BLUE}\uwave{#1}}} %
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                    
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{} 


==> zy_elem_ablation_num_frames.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{zz_figure_num_frames.pdf}
    \caption{Ablation over the maximum number of frames per sequence. We report the rank-1 accuracy for \colorbox{rgbexp!15}{RGB} and \colorbox{depthexp!15}{depth} and their corresponding standard error.}
    \label{fig:abl_num_frames}
\end{figure}


==> zy_elem_ablation_num_sequences.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{zz_figure_num_sequences.pdf}
    \caption{Ablation over the number of sequences in the gallery. We report the rank-1 accuracy for \colorbox{rgbexp!15}{RGB} and \colorbox{depthexp!15}{depth} and their corresponding standard error.}
    \label{fig:abl_num_sequences}
\end{figure}

